Not All Neuro-Symbolic Concepts Are Created Equal: Analysis and Mitigation of Reasoning Shortcuts

Neuro-Symbolic (NeSy) predictive models hold the promise of improved compliance with given constraints, systematic generalization, and interpretability, as they allow to infer labels that are consistent with some prior knowledge by reasoning over high-level concepts extracted from sub-symbolic inputs. It was recently shown that NeSy predictors are affected by reasoning shortcuts: they can attain high accuracy but by leveraging concepts with unintended semantics, thus coming short of their promised advantages. Yet, a systematic characterization of reasoning shortcuts and of potential mitigation strategies is missing. This work fills this gap by characterizing them as unintended optima of the learning objective and identifying four key conditions behind their occurrence. Based on this, we derive several natural mitigation strategies, and analyze their efficacy both theoretically and empirically. Our analysis shows reasoning shortcuts are difficult to deal with, casting doubts on the trustworthiness and interpretability of existing NeSy solutions.

==> tables/MTL_previous.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{lcccccccc}
\toprule
        & \multicolumn{8}{c}{Shortcut MNIST v2}                                                                                                                                                                                                                                                                        \\ \cmidrule(l){2-9} 
Task        & \multicolumn{2}{c}{DPL}                                                          &                          & \multicolumn{2}{c}{SL}                                                           &                          & \multicolumn{2}{c}{LTN}                                                          \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-9} 
        & F1 (Y)                                  & F1 (C)                                 &                          & F1 (Y)                                  & F1 (C)                                 &                          & F1 (Y)                                  & F1 (C)                                 \\
Add     & \cellcolor[HTML]{EFEFEF}$68.1 \pm 6.7$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.0$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.5 \pm 0.2$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$67.4 \pm 0.1$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.0$  \\
Mult    & $100.0 \pm 0.0$                         & $37.6 \pm 0.2$                         &                          & $100.0 \pm 0.0$                         & $76.1 \pm 11.7$                        &                          & $98.1 \pm 0.5$                          & $78.1 \pm 0.4$                         \\
Multiop & \cellcolor[HTML]{EFEFEF}$100.0 \pm 0.0$ & \cellcolor[HTML]{EFEFEF}$99.8 \pm 0.1$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$100.0 \pm 0.0$ & \cellcolor[HTML]{EFEFEF}$99.8 \pm 0.1$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}\bf $98.3 \pm 0.2$ & \cellcolor[HTML]{EFEFEF} \bf $98.3 \pm 0.2$ \\ \bottomrule
\end{tabular}


==> tables/SHORMNIST_previous.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{lcccccccc}
    \toprule
          & \multicolumn{8}{c}{\MNISTShortcut}                                                                                                                                                                                                                                                                                   \\ \cline{2-9} 
Mitigation& \multicolumn{2}{c}{DPL}                                                                  &                          & \multicolumn{2}{c}{SL}                                                          &                          & \multicolumn{2}{c}{LTN}                                                           \\ \cline{2-3} \cline{5-6} \cline{8-9} 
          & F1 (Y)                                          & F1 (C)                                 &                          & F1 (Y)                                 & F1(C)                                  &                          & F1 (Y)                                  & F1(C)                                   \\
None      & \cellcolor[HTML]{EFEFEF}$85.1 \pm 4.6$          & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.3 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$0.2 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} $ 98.1 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$0.3 \pm 0.1$   \\
R         & $79.8 \pm 1.0$                                  & $0.1 \pm 0.0$                          &                          & $99.5 \pm 0.2$                         & $0.1 \pm 0.0$                          &                          & $76.3 \pm 1.1$                          & $0.0 \pm 0.0$                           \\
H         & \cellcolor[HTML]{EFEFEF}$98.1 \pm 0.1$          & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.4 \pm 0.1$ & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.0$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$81.9 \pm 0.5$  & \cellcolor[HTML]{EFEFEF}$53.9 \pm 0.7$  \\
C         & ${84.9 \pm 0.1}$                         & $0.1 \pm 0.1$                         &                          & $99.3 \pm 0.4$                         & $21.5 \pm 6.2$                         &                          & ${98.1 \pm 0.2}$                & $0.2 \pm 0.1$                          \\
R + H     & \cellcolor[HTML]{EFEFEF}${75.4 \pm 0.4}$ & \cellcolor[HTML]{EFEFEF}$0.2 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.6 \pm 0.1$ & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.0$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$97.9 \pm 2.3$  & \cellcolor[HTML]{EFEFEF}$38.1 \pm 16.7$ \\
R + C     & ${84.0 \pm 2.2}$                         & $1.9 \pm 4.4$                         &                          & $99.3 \pm 0.2$                         & $61.5 \pm 7.8$                         &                          & ${ 98.1 \pm 0.2 }$                 & $0.2 \pm 0.1$                          \\
H + C     & \cellcolor[HTML]{EFEFEF}$91.9 \pm 3.5$          & \cellcolor[HTML]{EFEFEF}$88.0 \pm 6.3$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.4 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$41.5 \pm 8.2$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$98.2 \pm 0.2$  & \cellcolor[HTML]{EFEFEF}$98.6 \pm 0.1$  \\
R + H + C & $95.4 \pm 0.4$                                  & $96.2 \pm 0.2$                         &                          & $99.5 \pm 0.2$                         & $47.2 \pm 9.8$                         &                          & $98.1 \pm 0.3$                          & $98.5 \pm 0.2$                         \\
\bottomrule
\end{tabular}

==> tables/XOR_results_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%
%
%
% \begin{tabular}{lccccccccccc}
%     \toprule
%     & \multicolumn{5}{c}{\XOR}  &                         & \multicolumn{5}{c}{\MNISTAdd}
%     \\
%     \cline{2-6} \cline{8-12} 
%                                 & \multicolumn{1}{c}{DPL}   &         & \multicolumn{1}{c}{SL}   &                          & \multicolumn{1}{c}{LTN}  & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{DPL}  &                          & \multicolumn{1}{c}{SL}   &                          & \multicolumn{1}{c}{LTN}
%     \\ 
%     \rowcolor[HTML]{EFEFEF} --    & $100\%$                   &  &  $100\%$ &  &  $100\%$ &  &  $96.7\%$ &  &  $82.9\%$ &  &  $100\%$
%     \\
%     \DIS    &  $0\%$ &  &  $0\%$ &  &  $0\%$ &   &  $0\%$ &  &  $0\%$ &   & $0\%$  
%     \\
% \bottomrule
% \end{tabular}
%
%
%
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccccc}
    \toprule
    & \multicolumn{6}{c}{\XOR}            
    \\
    \cmidrule(lr){2-7} %\cmidrule(lr){5-7} 
                                & \multicolumn{2}{c}{DPL}                    &  \multicolumn{2}{c}{SL}                    & \multicolumn{2}{c}{LTN}  
    \\                          % DPL                                        % SL                                          % LTN
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
    & \textsc{Acc}($\vY$) & \textsc{Acc}($\vC$) & \textsc{Acc}($\vY$) & \textsc{Acc}($\vC$) & \textsc{Acc}($\vY$) & \textsc{Acc}($\vC$) & \\ 
    \rowcolor[HTML]{EFEFEF} --  & $ 80.6 \pm 16.9 \% $ & $22.0 \pm 7.1 \%$   &  $89.3  \pm 15.9 \% $ & $23.7 \pm 7.0 \%$   &  $83.9 \pm 14.5 \%$ & $ 20.5 \pm 9.0 \% $ 
    \\                          % DPL                                        % SL                                          % LTN 
    \DIS                        & $82.1 \pm 24.0 \%$ & $68.8 \pm 41.9 \%$    &  $84.2 \pm 21.6 \%$ & $82.5 \pm 35.0 \%$    & $93.3 \pm 17.0 \%$ & $88.8 \pm 28.8 \%$  
    \\
    \midrule \\
    %
    & \multicolumn{6}{c}{\MNISTAdd}            
    \\
    \cmidrule(lr){2-7} %\cmidrule(lr){5-7} 
                                & \multicolumn{2}{c}{DPL}                    &  \multicolumn{2}{c}{SL}                    & \multicolumn{2}{c}{LTN}  
    \\                          % DPL                                        % SL                                          % LTN
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
    & \textsc{Acc}($\vY$) & \textsc{Acc}($\vC$) & \textsc{Acc}($\vY$) & \textsc{Acc}($\vC$) & \textsc{Acc}($\vY$) & \textsc{Acc}($\vC$) & \\
    %
    \rowcolor[HTML]{EFEFEF} --  & $ 96.3 \pm 1.2 \% $ & $43.1 \pm 21.3 \% $    &  $ 97.0 \pm 0.3 \% $ & $ 40.2 \pm 26.3 \% $  &   $78.5 \pm 25.1 \%$ & $46.3 \pm 17.1 \%$ 
    \\                          % DPL                                          % SL                                            % LTN
    \DIS                        & $99.5 \pm 0.1 \% $ & $ 99.7 \pm 0.1 \%$    &  $98.8 \pm 0.1 \%$ & $ 99.7 \pm 0.1 \% $   & $ 95.8 \pm 5.5 \%  $ & $ 97.8 \pm 3.0 \% $  
    \\
\bottomrule
\end{tabular}

% MODEL:  mnistltn  joint: True
% Y:    78.46617247442455 +- 25.13541058193295  $78.5 \pm 25.1 \%$ & $46.3 \pm 17.1 \%$
% C:    46.31778492647059 +- 17.046635028912945
% MODEL:  mnistltn  joint: False
% Y:    95.82625679347827 +- 5.4975704052274565 $ 95.8 \pm 5.5 \%  $ & $ 97.8 \pm 3.0 \% $
% C:    97.81886888586958 +- 2.998523083000285

% MODEL:  mnistsl  joint: True
% Y:    96.97039175724636 +- 0.30750717785563325 $ 97.0 \pm 0.3 \% $ & $ 40.2 \pm 26.3 \% $ 
% C:    40.2432914402174 +- 26.34323442596824
% MODEL:  mnistsl  joint: False
% Y:    98.76188858695652 +- 0.07156701766447661 $98.8 \pm 0.1 \%$ & $ 99.7 \pm 0.1 \% $
% C:    99.7276947463768 +- 0.021781033291678697

% MODEL:  mnistdpl  joint: True
% Y:    96.3176517210145 +- 1.1659041799331722 
% C:    43.10702558876812 +- 21.282332956250276
% MODEL:  mnistdpl  joint: False
% Y:    99.45227581521735 +- 0.049793905619635995 $99.5 \pm 0.1 \% $ & $ 99.7 \pm 0.1 \%$
% C:    99.72599637681164 +- 0.024775571401871473


==> tables/analysis_XOR_complete.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{lccccccccccc}
    \toprule
    & \multicolumn{5}{c}{\XOR}  &                         & \multicolumn{5}{c}{\MNISTAdd}
    \\
    \cline{2-6} \cline{8-12} 
                                & \multicolumn{1}{c}{DPL}   &         & \multicolumn{1}{c}{SL}   &                          & \multicolumn{1}{c}{LTN}  & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{DPL}  &                          & \multicolumn{1}{c}{SL}   &                          & \multicolumn{1}{c}{LTN}
    \\ 
    \rowcolor[HTML]{EFEFEF} w/o \DIS    & $100\%$                   &  &  $100\%$ &  &  $100\%$ &  &  $96.7\%$ &  &  $82.9\%$ &  &  $100\%$
    \\
    w/ \DIS                             & $67.5\%$                &                          &           $68.5\%$               &                          & $61.5\%$                          &                         & $0\%$                         &                          &     $0\%$                     &                           &      $0\%$                    
    \\
    \rowcolor[HTML]{EFEFEF} w/ \DIS+\SW    &  $0\%$ &  &  $0\%$ &  &  $0\%$ &   &  $0\%$ &  &  $0\%$ &   & $0\%$  
    \\
\bottomrule
\end{tabular}

==> tables/results_BDD_OIA_complete.tex <==
\begin{tabular}{llllllllllll}
\toprule
                    & \multicolumn{10}{c}{BDD-OIA}                                                                                                                                                                                                                                               &  \\ \cline{2-11}
                    & \multicolumn{1}{c}{F1 (Forward)} & \multicolumn{1}{c}{F1 (Stop)} & \multicolumn{1}{c}{F1 (Left)} & \multicolumn{1}{c}{F1 (Right)} &  & \multicolumn{1}{c}{F1-mean (Y)} & \multicolumn{1}{c}{F1-mean(C)} &  & \multicolumn{1}{c}{F1-all(Y)} & \multicolumn{1}{c}{F1-all(C)} &  \\
C                & $ 0.739 \pm 0.002 $              & $ 0.771 \pm 0.002 $           & $ 0.474 \pm 0.008 $           & $ 0.607 \pm 0.003 $            &  & $0.648 \pm 0.002$               & $0.603 \pm 0.001$              &  & $0.663 \pm 0.003 $            & $0.719 \pm 0.001 $            &  \\
DPL             & $ 0.766 \pm 0.002 $              & $ 0.766 \pm 0.001 $           & $ 0.659 \pm 0.002 $           & $ 0.665 \pm 0.002 $            &  & $0.714 \pm 0.001$               & $0.394 \pm 0.062$              &  & $0.744 \pm 0.001 $            & $0.467 \pm 0.006 $            &  \\
DPL+C(FS)     & $ 0.766 \pm 0.002 $              & $ 0.767 \pm 0.002 $           & $ 0.660 \pm 0.002 $           & $ 0.665 \pm 0.002 $            &  & $0.715 \pm 0.008$               & $0.386 \pm 0.624$              &  & $0.744 \pm 0.001 $            & $0.464 \pm 0.006 $            &  \\
DPL+H           & $ 0.765 \pm 0.002 $              & $ 0.771 \pm 0.002 $           & $ 0.683 \pm 0.001 $           & $ 0.665 \pm 0.002 $            &  & $0.721 \pm 0.001$               & $0.481 \pm 0.003$              &  & $0.740 \pm 0.001 $            & $0.522 \pm 0.002 $            &  \\
DPL+C           & $ 0.753 \pm 0.002 $              & $ 0.765 \pm 0.001 $           & $ 0.570 \pm 0.008 $           & $ 0.639 \pm 0.002 $            &  & $0.682 \pm 0.002$               & $0.605 \pm 0.001$              &  & $0.709 \pm 0.002 $            & $0.721 \pm 0.001 $            &  \\
DPL+C+H        & $ 0.754 \pm 0.001 $              & $ 0.771 \pm 0.001 $           & $ 0.577 \pm 0.012 $           & $ 0.630 \pm 0.003 $            &  & $0.683 \pm 0.003$               & $0.617 \pm 0.001$              &  & $0.721 \pm 0.001 $            & $0.729 \pm 0.001 $            &  \\
\bottomrule
\end{tabular}

==> tables/results_BDD_OIA_incomplete.tex <==
\begin{tabular}{llllllll}
\toprule
                    & \multicolumn{7}{c}{\BOIA}                                                                                                                                                                             \\ \cline{2-8} 
                    & \multicolumn{1}{c}{F1 (Forward)} & \multicolumn{1}{c}{F1 (Stop)} & \multicolumn{1}{c}{F1 (Left)} & \multicolumn{1}{c}{F1 (Right)} &  & \multicolumn{1}{c}{F1-mean (Y)} & \multicolumn{1}{c}{F1-mean(C)} \\
CSUP                & $ 0.739 \pm 0.002 $              & $ 0.771 \pm 0.002 $           & $ 0.474 \pm 0.008 $           & $ 0.607 \pm 0.003 $            &  & $0.648 \pm 0.002$               & $0.603 \pm 0.001$              \\
DPL + K             & $ 0.766 \pm 0.002 $              & $ 0.766 \pm 0.001 $           & $ 0.659 \pm 0.002 $           & $ 0.665 \pm 0.002 $            &  & $0.714 \pm 0.001$               & $0.394 \pm 0.062$              \\
DPL + K + LCSUP     & $ 0.766 \pm 0.002 $              & $ 0.767 \pm 0.002 $           & $ 0.660 \pm 0.002 $           & $ 0.665 \pm 0.002 $            &  & $0.715 \pm 0.008$               & $0.386 \pm 0.624$              \\
DPL +K +H           & $ 0.765 \pm 0.002 $              & $ 0.771 \pm 0.002 $           & $ 0.683 \pm 0.001 $           & $ 0.665 \pm 0.002 $            &  & $0.721 \pm 0.001$               & $0.481 \pm 0.003$              \\
DPL +K +C           & $ 0.753 \pm 0.002 $              & $ 0.765 \pm 0.001 $           & $ 0.570 \pm 0.008 $           & $ 0.639 \pm 0.002 $            &  & $0.682 \pm 0.002$               & $0.605 \pm 0.001$              \\
DPL +K +C +H        & $ 0.754 \pm 0.001 $              & $ 0.771 \pm 0.001 $           & $ 0.577 \pm 0.012 $           & $ 0.630 \pm 0.003 $            &  & $0.683 \pm 0.003$               & $0.617 \pm 0.001$              \\
\bottomrule
\end{tabular}

==> tables/results_MULTITASK.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%
%
%
%
% \begin{tabular}{lcccccccc}
% \toprule
% Task        & \multicolumn{2}{c}{DPL}                                                          &                          & \multicolumn{2}{c}{SL}                                                           &                          & \multicolumn{2}{c}{LTN}                                                          \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-9} 
%         & F1 (Y)                                  & F1 (C)                                 &                          & F1 (Y)                                  & F1 (C)                                 &                          & F1 (Y)                                  & F1 (C)                                 \\
% \cellcolor[HTML]{EFEFEF}\textsc{Add}     & \cellcolor[HTML]{EFEFEF}$68.1 \pm 6.7$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.0$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.5 \pm 0.2$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$67.4 \pm 0.1$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.0$  \\
% \textsc{Mult}    & $100.0 \pm 0.0$                         & $37.6 \pm 0.2$                         &                          & $100.0 \pm 0.0$                         & $76.1 \pm 11.7$                        &                          & $98.1 \pm 0.5$                          & $78.1 \pm 0.4$                         \\
% \cellcolor[HTML]{EFEFEF}\textsc{MultiOp} & \cellcolor[HTML]{EFEFEF}$100.0 \pm 0.0$ & \cellcolor[HTML]{EFEFEF}$99.8 \pm 0.1$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$100.0 \pm 0.0$ & \cellcolor[HTML]{EFEFEF}$99.8 \pm 0.1$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}\bf $98.3 \pm 0.2$ & \cellcolor[HTML]{EFEFEF} \bf $98.3 \pm 0.2$ \\ \bottomrule
% \end{tabular}
%
%
% WE CAN WRITE A/ M / A+M to save space. al posto di add, mul and multiop
\setlength{\tabcolsep}{3pt}
\scalebox{.9}{
\begin{tabular}{lcccccc}
\toprule
Task        & \multicolumn{2}{c}{DPL}                                                                          & \multicolumn{2}{c}{SL}                                                                             & \multicolumn{2}{c}{LTN}                                                          \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7} 
        & F1 (Y)                                  & F1 (C)                                                       & F1 (Y)                                  & F1 (C)                                 &                           F1 (Y)                                  & F1 (C)                                 \\
\cellcolor[HTML]{EFEFEF}\textsc{Add}     & \cellcolor[HTML]{EFEFEF}$68.1 \pm 6.7$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.0$  &  \cellcolor[HTML]{EFEFEF}$99.5 \pm 0.2$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.1$  &  \cellcolor[HTML]{EFEFEF}$67.4 \pm 0.1$  & \cellcolor[HTML]{EFEFEF}$0.0 \pm 0.0$  \\
\textsc{Mult}    & $100.0 \pm 0.0$                         & $37.6 \pm 0.2$                                                 & $100.0 \pm 0.0$                         & $76.1 \pm 11.7$                        &                           $98.1 \pm 0.5$                          & $78.1 \pm 0.4$                         \\
\cellcolor[HTML]{EFEFEF}\textsc{MultiOp} & \cellcolor[HTML]{EFEFEF}$100.0 \pm 0.0$ & \cellcolor[HTML]{EFEFEF}$99.8 \pm 0.1$ &  \cellcolor[HTML]{EFEFEF}$100.0 \pm 0.0$ & \cellcolor[HTML]{EFEFEF}$99.8 \pm 0.1$ &  \cellcolor[HTML]{EFEFEF}\bf $98.3 \pm 0.2$ & \cellcolor[HTML]{EFEFEF} \bf $98.3 \pm 0.2$ \\ \bottomrule
\end{tabular}
}


==> tables/results_SHORTMNIST.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

%
%
%
% \begin{tabular}{lcccccccc}
%     \toprule
% Mitigation& \multicolumn{2}{c}{DPL}                                                                  &                          & \multicolumn{2}{c}{SL}                                                          &                          & \multicolumn{2}{c}{LTN}                                                           \\ \cline{2-3} \cline{5-6} \cline{8-9} 
%           & F1 (Y)                                          & F1 (C)                                 &                          & F1 (Y)                                 & F1(C)                                  &                          & F1 (Y)                                  & F1(C)                                   \\
% \cellcolor[HTML]{EFEFEF}--      & \cellcolor[HTML]{EFEFEF}$85.1 \pm 4.6$          & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.3 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$0.2 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} $ 98.1 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$0.3 \pm 0.1$   \\
% \MSR         & $79.8 \pm 1.0$                                  & $0.1 \pm 0.0$                          &                          & $99.5 \pm 0.2$                         & $0.1 \pm 0.0$                          &                          & $76.3 \pm 1.1$                          & $0.0 \pm 0.0$                           \\
% \cellcolor[HTML]{EFEFEF}\MSH         & \cellcolor[HTML]{EFEFEF}$98.1 \pm 0.1$          & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.4 \pm 0.1$ & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.0$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$81.9 \pm 0.5$  & \cellcolor[HTML]{EFEFEF}$53.9 \pm 0.7$  \\
% \MSC         & ${84.9 \pm 0.1}$                         & $0.1 \pm 0.1$                         &                          & $99.3 \pm 0.4$                         & $21.5 \pm 6.2$                         &                          & ${98.1 \pm 0.2}$                & $0.2 \pm 0.1$                          \\
% \cellcolor[HTML]{EFEFEF}\MSR + \MSH     & \cellcolor[HTML]{EFEFEF}${75.4 \pm 0.4}$ & \cellcolor[HTML]{EFEFEF}$0.2 \pm 0.1$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.6 \pm 0.1$ & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.0$  & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$97.9 \pm 2.3$  & \cellcolor[HTML]{EFEFEF}$38.1 \pm 16.7$ \\
% \MSR + \MSC     & ${84.0 \pm 2.2}$                         & $1.9 \pm 4.4$                         &                          & $99.3 \pm 0.2$                         & $61.5 \pm 7.8$                         &                          & ${ 98.1 \pm 0.2 }$                 & $0.2 \pm 0.1$                          \\
% \cellcolor[HTML]{EFEFEF}\MSH + \MSC     & \cellcolor[HTML]{EFEFEF}$91.9 \pm 3.5$          & \cellcolor[HTML]{EFEFEF}$88.0 \pm 6.3$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$99.4 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$41.5 \pm 8.2$ & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}$98.2 \pm 0.2$  & \cellcolor[HTML]{EFEFEF}$98.6 \pm 0.1$  \\
% \MSR + \MSH + \MSC & $95.4 \pm 0.4$                                  & $96.2 \pm 0.2$                         &                          & $99.5 \pm 0.2$                         & $47.2 \pm 9.8$                         &                          & $98.1 \pm 0.3$                          & $98.5 \pm 0.2$                         \\
% \bottomrule
% \end{tabular}
%
%
%
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccccc}
    \toprule
Mitigation & \multicolumn{2}{c}{DPL}                                                                  &                          \multicolumn{2}{c}{SL}                                                                                   & \multicolumn{2}{c}{LTN}                                                           \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
          & F1 (Y)                                          & F1 (C)                                                          & F1 (Y)                                 & F1(C)                                                           & F1 (Y)                                  & F1(C)                                   \\
\cellcolor[HTML]{EFEFEF}--      & \cellcolor[HTML]{EFEFEF}$85.1 \pm 4.6$          & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.1$  & \cellcolor[HTML]{EFEFEF}$99.3 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$0.2 \pm 0.1$   & \cellcolor[HTML]{EFEFEF} $ 98.1 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$0.3 \pm 0.1$   \\
\MSR         & $79.8 \pm 1.0$                                  & $0.1 \pm 0.0$                                         & $99.5 \pm 0.2$                         & $0.1 \pm 0.0$                                                   & $76.3 \pm 1.1$                          & $0.0 \pm 0.0$                           \\
\cellcolor[HTML]{EFEFEF}\MSH         & \cellcolor[HTML]{EFEFEF}$98.1 \pm 0.1$          & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.1$  &  \cellcolor[HTML]{EFEFEF}$99.4 \pm 0.1$ & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.0$  &  \cellcolor[HTML]{EFEFEF}$81.9 \pm 0.5$  & \cellcolor[HTML]{EFEFEF}$53.9 \pm 0.7$  \\
\MSC         & ${84.9 \pm 0.1}$                         & $0.1 \pm 0.1$                                               & $99.3 \pm 0.4$                         & $21.5 \pm 6.2$                                                & ${98.1 \pm 0.2}$                & $0.2 \pm 0.1$                          \\
\cellcolor[HTML]{EFEFEF}\MSR + \MSH     & \cellcolor[HTML]{EFEFEF}${75.4 \pm 0.4}$ & \cellcolor[HTML]{EFEFEF}$0.2 \pm 0.1$   & \cellcolor[HTML]{EFEFEF}$99.6 \pm 0.1$ & \cellcolor[HTML]{EFEFEF}$0.1 \pm 0.0$  &  \cellcolor[HTML]{EFEFEF}$97.9 \pm 2.3$  & \cellcolor[HTML]{EFEFEF}$38.1 \pm 16.7$ \\
\MSR + \MSC     & ${84.0 \pm 2.2}$                         & $1.9 \pm 4.4$                                               & $99.3 \pm 0.2$                         & $61.5 \pm 7.8$                                                & ${ 98.1 \pm 0.2 }$                 & $0.2 \pm 0.1$                          \\
\cellcolor[HTML]{EFEFEF}\MSH + \MSC     & \cellcolor[HTML]{EFEFEF}$91.9 \pm 3.5$          & \cellcolor[HTML]{EFEFEF}$88.0 \pm 6.3$ &  \cellcolor[HTML]{EFEFEF}$99.4 \pm 0.2$ & \cellcolor[HTML]{EFEFEF}$41.5 \pm 8.2$ &  \cellcolor[HTML]{EFEFEF}$98.2 \pm 0.2$  & \cellcolor[HTML]{EFEFEF}$98.6 \pm 0.1$  \\
\MSR + \MSH + \MSC & $95.4 \pm 0.4$                                  & $96.2 \pm 0.2$                                                   & $99.5 \pm 0.2$                         & $47.2 \pm 9.8$                         &                           $98.1 \pm 0.3$                          & $98.5 \pm 0.2$                         \\
\bottomrule
\end{tabular}

==> tables/results_XOR.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{lllllllll}
\toprule
Mitigation & \multicolumn{8}{c}{XOR}  \\ \cline{2-9} 
           & \multicolumn{2}{c}{DPL}                             &                          & \multicolumn{2}{c}{SL}                              &                          & \multicolumn{2}{c}{LTN}                             \\ \cline{2-3} \cline{5-6} \cline{8-9} 
           & Acc (Y)                  & Acc (C)                  &                          & Acc (Y)                  & Acc (C)                  &                          & Acc (Y)                  & Acc (C)                  \\
None       & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} \\
R          &                          &                          &                          &                          &                          &                          &                          &                          \\
H          & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} \\
C          &                          &                          &                          &                          &                          &                          &                          &                          \\
R + H      & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} \\
R + C      &                          &                          &                          &                          &                          &                          &                          &                          \\
H + C      & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} \\
R + H + C  &                          &                          &                          &                          &                          &                          &                          &                          \\
\bottomrule            
\end{tabular}


==> tables/results_XOR_SHORTMNIST.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{llllllllllllll}
\toprule
Mitigation & \multicolumn{6}{c}{XOR}                                                                                      &  & \multicolumn{6}{c}{SHORT-MNIST}                                                                              \\ \cline{2-7} \cline{9-14} 
           & \multicolumn{2}{c}{DPL}            & \multicolumn{2}{c}{SL}             & \multicolumn{2}{c}{LTN}            &  & \multicolumn{2}{c}{DPL}            & \multicolumn{2}{c}{SL}             & \multicolumn{2}{c}{LTN}            \\
           & Acc (Y) & Acc (C)                  & Acc (Y) & Acc (C)                  & Acc (Y) & Acc (C)                  &  & Acc (Y) & Acc (C)                  & Acc (Y) & Acc (C)                  & Acc (Y) & Acc (C)                  \\
None       &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
R          &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
H          &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
C          &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
R + H      &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
R + C      &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
H + C      &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
R + H + C  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &  &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} &         & \cellcolor[HTML]{EFEFEF} \\
\bottomrule
\end{tabular}
